Robust Safety-Critical Control for Dynamic Robotics

We present a novel method of optimal robust control through quadratic programs that offers tracking stability while subject to input and state-based constraints as well as safety-critical constraints for nonlinear dynamical robotic systems in the presence of model uncertainty. The proposed method formulates robust control Lyapunov and barrier functions to provide guarantees of stability and safety in the presence of model uncertainty. We evaluate our proposed control design on dynamic walking of a five-link planar bipedal robot subject to contact force constraints as well as safety-critical precise foot placements on stepping stones, all while subject to model uncertainty. We conduct preliminary experimental validation of the proposed controller on a rectilinear spring-cart system under different types of model uncertainty and perturbations.

==> adverse_effect.tex <==
\section{Adverse Effects of Uncertainty in Dynamics on the CBF-CLF-QP controller}
\label{sec:adverse_effect}

The controller presented in Section \ref{sec:CLF_CBF_revisited} provide means of an optimal control scheme that balances conflicting requirements between stability, state-based constraints and energy consumption. It is a powerful method that has been deployed successfully for different applications, for example Adaptive Cruise Control \cite{CBF:Ames:ExperimentalACC:ACC15}, quadrotor flight \cite{CBF:Guofan:SafetyCriteria:ACC15}, and dynamic walking for bipedal robots \cite{CBF:Quan:Footstep:ADHS15}, \cite{CBF:Ames:CBFBiped:ACC15}.

However, a  primary disadvantage of the CBF-CLF-QP controller is that it requires the knowledge of an accurate dynamical model of the plant to make guarantees on stability as well as safety. In particular, enforcing the CLF and CBF conditions in the QP \eqref{CBF_CLF_QP_controller} requires the accurate knowledge of the nonlinear dynamics $f(x), g(x)$ to compute the Lie derivatives in \eqref{lie_deriv_ddy_fg}, \eqref{LfVLgVdefns2} and \eqref{lie_deriv_dB_fg}. Therefore, model uncertainty that is usually present in physical systems can potentially cause poor quality of control leading to tracking errors, and lead to instability \cite{NgSr2014Robust_RSS}, as well as violation of the safety-critical constraints \cite{CBF:Ames:RobustnessCBF:ADHS15}.  In this section, we will explore the effect of uncertainty on the CLF-QP controller, input and state constraints, and safety constraints enforced by the CBF-QP controller.

\subsection{Effects of uncertainty on CLFs}
\begin{table}
\centering
\begin{tabular}{ |c|c|c| } 
	\hline
	Notations & Model types\\
	\hline
	{\large $f,g$} & true nonlinear model\\ 
	%\hline
	{\large $\tilde{f}, \tilde{g}$} & nominal nonlinear model\\ 
	%\hline
	{\large $\bar f, \bar g$} & true I-O linearized model\\
	%\hline
	{\large $\tilde{\bar f}, \tilde{\bar g}$} & nominal I-O linearized model \\
	\hline
\end{tabular}
\caption{A list of notations for different models used in this paper. A true model represents the actual (possibly not perfectly known) model of the physical system, while the nominal model represents the model that the controller uses.  While most controllers assume the true model is known, the robust controllers in this paper use the nominal models and offer robustness guarantees to the uncertainty between the two models.}
	\label{tab:ModelTypes}
\end{table}

In order to analyze the affect of model uncertainty in our controllers, we assume that the vector fields, $f(x), g(x)$ of the real dynamics \eqref{fg_affine}, are unknown. We therefore have to design our controller based on the nominal vector fields $\tilde{f}(x), \tilde{g}(x)$.  Then, the pre-control law \eqref{expControl} get's reformulated as 
\begin{equation}
\label{preControlUncertainty}
u(x) = \tilde u_{ff}(x) + (L_{\tilde{g}}L_{\tilde{f}} y(x))^{-1}\mu,
%u(q,\dot{q}) = u^{*}(q,\dot{q})+\mu
\end{equation}
with
\begin{equation}
\label{ustarUncertainty}
	\tilde u_{ff}(x) := -(L_{\tilde{g}}L_{\tilde{f}} y(x))^{-1} L^2_{\tilde{f}} y(x),
\end{equation}
where we have used the nominal model rather than the unknown real dynamics.

Substituting $ u(x) $ from \eqref{preControlUncertainty} into \eqref{linearied_output_h}, the input-output linearized system then becomes
\begin{equation}
\label{yddotUncertainty}
\ddot y = \mu+\Delta_{1}+\Delta_{2}\mu,
%\ddot{y} = \mu+\Delta_{1},
\end{equation}
where $\Delta_1 \in \mathbb{R}^m, \Delta_2 \in \mathbb{R}^{m\times m}$, are given by,
\begin{align}
\label{DeltaUncertainty}
\Delta_{1}&:=L^2_{f}h(x)-L_{g}L_{f} h(x)(L_{\tilde{g}}L_{\tilde{f}} h(x))^{-1}L^2_{\tilde{f}}h(x),  \nonumber\\
\Delta_{2}&:=L_{g}L_{f} h(x)(L_{\tilde{g}}L_{\tilde{f}} h(x))^{-1}-I.
\end{align}
\begin{remark}
	In the definitions of $\Delta_1, \Delta_2$, note that when there is no model uncertainty, i.e., $\tilde{f}=f, \tilde{g}=g$, then $\Delta_1 = \Delta_2 = 0$.
\end{remark}

Using $F$ and $G$ as in \eqref{FGdefns}, the closed-loop system now takes the form
\begin{equation}
\label{EtaClosedLoopUncertainty}
\dot{\eta}=F\eta+\begin{bmatrix} O \\ \Delta_1 
\end{bmatrix}+(G+\begin{bmatrix} O \\ \Delta_2 
\end{bmatrix})\mu.
%\dot{\eta}=F\eta+G\mu+\Delta H.
\end{equation}
 
In fact for $\Delta_1 \ne 0$, the closed-loop system does not have an equilibrium, and for $\Delta_2 \ne 0$, the controller could potentially destabilize the system (see \cite{reed1989instability}).
This raises the question of whether it's possible for controllers to account for this model uncertainty, and if so, how do we design such a controller. In particular, the time-derivative of the CLF in \eqref{eq:CLF_time_deriv} becomes more complex and dependent on $\Delta_1, \Delta_2$.

Notice that the robust RES condition in \eqref{eq:robust_RES_cond} is affine in the control inputs $\mu$ and thus can be expressed as
\begin{equation}
\label{RESIneqUncertainty}
\max_{\substack{||\Delta_1||\le \Delta_1^{max} \\ ||\Delta_2||\le \Delta_2^{max} }} {\Psi}_{0}+{\Psi}_{1}\mu \le 0,
\end{equation}
where
\begin{align}
\label{TildePsi01Defns}
{\Psi}_{0}(\eta, \Delta_1)&:= L_{\bar{f}}V_\epsilon(\eta)%\etavar^T (F^T P_{\epsilon} + P_{\epsilon} F) \etavar + 2 \eta ^T P_{\epsilon} \Delta H 
+ \frac{c_3}{\epsilon}V_{\epsilon},\nonumber\\
{\Psi}_{1}(\eta, \Delta_2) &:= L_{\bar{g}}V_\epsilon(\eta),%2 \etavar^T P_{\epsilon} (G+ \Delta G).
\end{align}
with $L_{\bar{f}}V_\epsilon(\eta), L_{\bar{g}}V_\epsilon(\eta)$ as defined in \eqref{BarLfVandLgVUncertainty}.

The goal of the robust control design is then to find the control $\mu$ satisfying the RES condition \eqref{RESIneqUncertainty}, evaluated through the given bounds of uncertainty in \eqref{assump:BoundUncertainty}. However, our controller can only use the nominal model $\tilde{\bar f}, \tilde{\bar g}$ and not the true model $\bar f, \bar g$ (see Table \ref{tab:ModelTypes} for different types of models).  We thus define the Lie derivatives of $V$ with respect to the nominal model as
\begin{align}
L_{\tilde {\bar f}}V&=\etavar^T (F^T P_{\epsilon} + P_{\epsilon} F) \etavar, \\
L_{\tilde {\bar g}}V&=2 \etavar^T P_{\epsilon} G.
\end{align}

Then, from \eqref{BarLfVandLgVUncertainty}, we have
\begin{align}
\dot V &= L_{\bar f} V + L_{\bar g}V \mu \\
& = L_{\tilde{\bar f}}V 
+ \underbrace{2\eta ^T P_{\epsilon} \begin{bmatrix}\textbf{0}\\\Delta_1\end{bmatrix} }_{\Delta_1^v} 
+ \underbrace{L_{\tilde{\bar g}}V \mu}_{\mu_v} 
+ \underbrace{L_{\tilde {\bar g}}\Delta_2 \mu }_{\Delta_2^v \mu_v}\\
& =L_{\tilde {\bar f}}V + \Delta_1^v + (1 + \Delta_2^v) \mu_v,
\end{align}
where we have defined the following new scalar variables: uncertainty $\Delta_1^v \in \mathbb{R}$, control input $\mu_v \in \mathbb{R}$, and uncertainty $\Delta_2^v\in \mathbb{R}$.

Since $\Delta_1^v$ is the model uncertainty on $L_{\bar f}V$ and $\Delta_2^v$ is the model uncertainty on the mapping of the control input $\mu_v$, we then can simply design robust CLF condition using the assumption on the bounds of $\Delta_1^v$ and $\Delta_2^v$:
\begin{align}
||\Delta_1^v|| \le \Delta_{1,max}^v\\
||\Delta_2^v|| \le \Delta_{2,max}^v
\end{align}

We can then express \eqref{eq:robust_CLF_cond} as the following QP: 
%\todo{(Please update all the other QPs to have a similar format as this one using mytag\{\})}
\HRule
\noindent \textbf{Robust CLF-QP}:
%\begin{equation}
%\label{robust_CBF_QP}
%\begin{aligned}
%& \underset{\mu, \mu_b, d}{\argmin} & & \mu^T \mu + pd^2\\
%& \text{s.t.} & & \max_{\substack{||\Delta G||\le \Delta G_{max} \\ ||\Delta H||\le \Delta H_{max} }} \dot V_{\epsilon} (\eta, \Delta G, \Delta H, \mu) + \frac{c_3}{\epsilon}V_{\epsilon} \le d,\\
%&&&\max_{\substack{||\Delta_1^b||\le \Delta^b_{1,max} \\ ||\Delta_2^b||\le \Delta^b_{2,max} }} \dot B (x, \Delta_1^b, \Delta_2^b, \mu_b)-\frac{\gamma}{B(x)}\le 0\\
%&&& A_b(x)\mu+b_b(x)=\mu_b\\
%\end{aligned}
%\end{equation}
\begin{align} \label{robust_CLF}
u^*(x)=	& \underset{u,\mu,\mu_b,\delta }{\argmin} & & \mu^T \mu + p\delta^2 \\
& \text{s.t.} &&\max_{\substack{||\Delta_1^v||\le \Delta^v_{1,max} \\ ||\Delta_2^v||\le \Delta^v_{2,max} }} \dot V (x, \Delta_1^v, \Delta_2^v, \mu_b)-\frac{\gamma}{V(x)}\le 0, \nonumber \\
&&& L_{\tilde{f}}V(x)+L_{\tilde{g}}V(x)u=\mu_v, \mytag{Robust CLF} \\
&&& u =\tilde u_{ff}(x) + (L_{\tilde{g}} L_{\tilde{f}} y(x))^{-1} \mu. \mytag{IO}
\end{align}
\HRule

Therefore, the RES condition \eqref{RESIneqUncertainty} will hold if the following inequalities hold
\begin{align}
%\label{RESwithUncertaintyBoundCondition}
{\Psi}_{0}^{ max}+{\Psi}_{1}^p \mu \le 0, \nonumber \\
{\Psi}_{0}^{ max}+{\Psi}_{1}^n \mu \le 0,
\end{align}
where
\begin{align}
{\Psi}_{0}^{max}&= L_{\tilde{\bar f}}V+\frac{c_3}{\epsilon}V_{\epsilon}+||2 \eta ^T P_{\epsilon} \begin{bmatrix}\mathbf{0} \\ \mathbf{1} \end{bmatrix} ||\Delta_1^{max},\nonumber\\
{\Psi}_{1}^p& = L_{\tilde {\bar g}}V(1+\Delta_2^{max}),\nonumber\\
{\Psi}_{1}^n& =L_{\tilde {\bar g}}V(1-\Delta_2^{max}).
\end{align}
Thus the robust CLF-QP in \eqref{robust_CLF_QP} is then equivalent to the following optimization problem, which can clearly be seen as a QP:%We can then incorporate these inequalities into a new relaxed CLF-QP as follows:
%
%\HRule
%
%\noindent Robust CLF-QP:
\begin{align}
\label{cvxWithUncertainty}
\mu^* =& \underset{\mu}{\argmin} & & \mu^T \mu \\
& \text{s.t.} & & {\Psi}_{0}^{max}(\eta,\Delta_1^{max}) + {\Psi}_{1}^p(\eta,\Delta_2^{max})~\mu \le 0, \nonumber\\ & & & {\Psi}_{0}^{max}(\eta,\Delta_1^{max}) + {\Psi}_{1}^n(\eta,\Delta_2^{max})~\mu \le 0. \nonumber
\end{align}
Incorporating the above robust CLF constraint we have the following Robust CLF-QP with constraints:
\HRule
\noindent \textbf{Robust CLF-QP with Constraints}:
\begin{align}
\label{Robust_CBF_CLF_QP_form}
u^*(x)=& \underset{u,\mu, \delta_1, \delta_2}{\argmin} & & \mu^T \mu + p_1 \delta_1 ^2 + p_2 \delta_2^2\\
& \text{s.t.} & & {\Psi}_{0}^{max}(\eta,\Delta_1^{max}) + {\Psi}_{1}^p(\eta,\Delta_2^{max})~\mu \le \delta_1, \nonumber\\ 
& & & {\Psi}_{0}^{max}(\eta,\Delta_1^{max}) + {\Psi}_{1}^n(\eta,\Delta_2^{max})~\mu \le \delta_2. \nonumber \mytag{Robust CLF}\\
&&& A_c(x)u \le b_c(x), \nonumber \mytag{Constraints}\\
&&& u =u_{ff}(x) + (L_g L_f y(x))^{-1} \mu. \mytag{IO}
\end{align}
\HRule
The above can be represented in a similar form to \eqref{CLF_QP_form}, thus representing a quadratic program.
\subsection{Effect of uncertainty on constraints}
\label{subsec:uncertainty_constraints}
As developed in Section \ref{sec:CLF_CBF_revisited}, the input and state constraints can be expressed as \eqref{eq:constraints_u}.  These constraints depend on the model explicitly and are constraints on the real system dynamics.  We can thus rewrite the constraints showing explicit model dependence as,
%Constraint from the real model:
\begin{align} \label{eq:constraint_true_model}
A_c(x,f,g) u \le b_c(x,f,g).
\end{align}
If a controller naively enforces these constraints using the nominal model available to the controller, the controller will enforce the constraint
%Constraint computed from the nominal model
\begin{align}
\label{input_constraint_nominal_model}
A_c(x,\tilde{f},\tilde{g}) u \le b_c(x,\tilde{f},\tilde{g}).
\end{align}
that is different from the desired constraint we want to enforce on the real model \eqref{eq:constraint_true_model}.  For instance, to enforce a contact force constraint, if the controller computes and enforces the contact force constraint using the nominal model, there is absolutely no guarantee that the actual contact force on the real system satisfies the constraint.

\begin{remark}
	It must be noted that certain constraints do not depend on the model at all.  In such cases, model uncertainty does not affect the constraint.  One example of such a constraint is a pure input constraint, such as $u(x) \le u_{max}$.  Expressing this constraint in the form of \eqref{eq:constraint_true_model} results in $A_c = I, b_c = u_{max}$, which clearly is not dependent on the model.
\end{remark}


\subsection{Effects of uncertainty on CBFs}
\label{subsec:uncertainty_CBF}
Similar to what we have seen about the effect of uncertainty on CLFs and constraints, we will now see the effect of uncertainty on CBFs. We note that the time-derivative of the Barrier function in \eqref{CBF_candidate_inv} depends on the real model. Therefore we need to enforce the following constraint given by \eqref{eq:Bdot}:
\begin{align}
\label{CBF_cond_real}
\dot B(x,f,g,u)=\frac{\partial B}{\partial x}(f(x)+g(x)u)\le \frac{\gamma}{B(x)}
\end{align}
where $\dot x=f(x)+g(x)u$ is the real system dynamic.
As seen in the case of control Lyapunov functions and constraints, naively enforcing this barrier constraint using the nominal model results in,
\begin{align}
\label{CBF_cond_nominal_model}
\frac{\partial B}{\partial x}(\tilde f(x)+\tilde g(x)u)\le \frac{\gamma}{B(x)}
\end{align}
where $\dot x=\tilde f(x)+\tilde g(x)u$ is the nominal system dynamic known by the controller.
Clearly due to model uncertainty, or the significant difference between $(f(x),g(x))$ and $(\tilde f(x), \tilde g(x))$, this constraint is different from the previous one.  In fact, as analyzed in \cite{CBF:Ames:RobustnessCBF:ADHS15}, this results in violation of the safety-critical constraint established by the Barrier function.

\begin{remark}
	\label{rm:uncertainty_constraint}
	
With the CLF, the continuous-dynamics of \eqref{eq:lineaized_sys} is a linear time-invariant system ($F$ and $G$ are constant matrices), and thus we can evaluate the effect of uncertainty based on the difference with the static nominal model of $F$ and $G$ to obtain \eqref{EtaClosedLoopUncertainty}. However, in the case of constraints \eqref{input_constraint_nominal_model} and CBFs \eqref{CBF_cond_nominal_model}, the relation with the control input is not static (nonlinearly dependent on the system state $x$), and thus the same approach to analyze and explore the effect of model uncertainty as on CLFs could encounter difficulties. In order to solve this issue, we will introduce an alternative design of Virtual Input-Output Linearization that will help us to develop a novel method of Robust CBF-CLF-QP in the next section.
\end{remark}



